Automated Two Higgs Doublet Model at NLO

The Two Higgs Doublet Model at NLO is generated automatically by FeynRules and NLOCT and allows any computation to be performed at NLO in QCD inside MadGraph5_aMC@NLO. The model can handle both four and five massless flavours. Preliminary results of the shape comparison between the two schemes are shown.

==> preprint.tex <==
IPPP/14/109 , DCPT/14/218

